Symbolic Comparison of Geometric Quantities in GeoGebra

Comparison of geometric quantities usually means obtaining generally true equalities of different algebraic expressions of a given geometric figure. Today's technical possibilities already support symbolic proofs of a conjectured theorem, by exploiting computer algebra capabilities of some dynamic geometry systems as well. We introduce GeoGebra's new feature, the Compare command, that helps the users in experiments in planar geometry. We focus on automatically obtaining conjectures and their proofs at the same time, including not just equalities but inequalities too. Our contribution can already be successfully used to support teaching geometry classes at secondary level, by getting several well-known and some previously unpublished result within seconds on a modern personal computer.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2021 (ThEdu'21)\\
EPTCS 354, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.354.2}{10.4204/EPTCS.354.2}}
\pdfoutput=1

